PoroTwin: A digital twin for a FluidFlower rig

We present a framework for integrated experiments and simulations of tracer transport in heterogeneous porous media using digital twin technology. The physical asset in our setup is a meter-scale FluidFlower rig. The digital twin consists of a traditional physics-based forward simulation tool and a correction technique which compensates for mismatches between simulation results and observations. The latter augments the range of the physics-based simulation and allows us to bridge the gap between simulation and experiments in a quantitative sense. We describe the setup of the physical and digital twin, including data transfer protocols using cloud technology. The accuracy of the digital twin is demonstrated on a case with artificially high diffusion that must be compensated by the correction approach, as well as by simulations in geologically complex media. The digital twin is then applied to control tracer transport by manipulating fluid injection and production in the experimental rig, thereby enabling two-way coupling between the physical and digital twins.

==> junk/costa.tex <==


\begin{figure}[t]
\centering
    \includegraphics[width=\textwidth]{figures/DTporo2.pdf}
\caption{HAM: CoSTA}
\label{fig:dt1}
\end{figure}

In this section we present a brief justification of the use of CoSTA. It is based on the more thorough argument that can be found in~\cite{blakseth2022dnn}.
    
Consider the differential equation 

where $L_{\Omega}, L_{\partial \Omega}$ are differential operators, $f$ is a source term and $g$
a function specifying the boundary condition.
\begin{equation}
    L_{\Omega} = \phi \frac{\partial}{\partial t} + \nabla\cdot \mathbf{q}
\end{equation}
Now let $\tilde{u}$ be the solution to the perturbed problem
\begin{align}
    \tilde{L}_{\Omega}\tilde{u}&=\tilde{f}, \quad \forall \ x \in \Omega \nonumber\\
    \tilde{L}_{\partial \Omega} \tilde{u}&=\tilde{g} \quad \forall \ x \in \partial \Omega,
    \label{eq:perturbed_PDE}
\end{align}
where the perturbations $\tilde{\cdot}$ are due to imperfections such as unknown physics, modelling errors, discretization error, or inaccurate data. For example, we will later in this article simplify a nonlinear operator $L_\Omega$ with a linear (and discretized) $\tilde{L}_{\Omega}$.
Assume we can calculate the residuals defined as
\begin{align}
    r_{\Omega} &= \tilde{L}_{\Omega}(u-\tilde{u}) \nonumber\\
    r_{\partial \Omega} &=\tilde{L}_{\partial \Omega}(u-\tilde{u}),
\end{align}
and let $\hat{\tilde{u}}$ be the solution of the corrected, perturbed problem
\begin{align}
    \tilde{L}_{\Omega}\hat{\tilde{u}}&=\tilde{f}+r_{\Omega}, \quad \forall \ x \in \Omega \nonumber
    \\
    \tilde{L}_{\partial \Omega} \hat{\tilde{u}}&=\tilde{g}+r_{\partial \Omega}  \quad \forall \ x \in \partial \Omega.
    \label{eq:corrected_PDE}
\end{align}
Using the definition of the residuals, as well as the perturbed Equation~\eqref{eq:perturbed_PDE}, we see that 
\begin{align*}
    \tilde{L}_{\Omega}\hat{\tilde{u}}&=\tilde{f}+\tilde{L}_{\Omega}(u-\tilde{u}) = \tilde{L}_{\Omega}u, \quad \forall \ x \in \Omega\\
    \tilde{L}_{\partial \Omega} \hat{\tilde{u}}&=\tilde{g}+\tilde{L}_{\partial \Omega}(u-\tilde{u}) = \tilde{L}_{\partial \Omega}u  \quad \forall \ x \in \partial \Omega,
\end{align*}
which reduces to $\hat{\tilde{u}}=u$ if the corrected, perturbed problem~\eqref{eq:corrected_PDE} 
yields a unique solution.
From this argument, we see that the source term corrections are able to compensate for perturbations in the differential operators as well as the source terms.

In real scenarios, we obviously cannot calculate the residual exactly, as that would require the solution we are trying to estimate. The idea of the CoSTA method is to use a DDM to estimate the residual. For the input of the DDM we use the uncorrected solution $\tilde{u}$. This means the PBM is used twice, first to solve Equation~\eqref{eq:perturbed_PDE} for $\tilde{u}$, then Equation~\eqref{eq:corrected_PDE} for $\hat{\tilde{u}}$.
Since the DDM output is but a correction, the CoSTA framework exploits the knowledge in the physical model, unlike a pure DDM approach.


For the discretized version of heat equation derived in section~??, the corrected equation is
\begin{equation}
    (M+kA)(\boldsymbol{u_i})=M\boldsymbol{u_{i-1}} + F_i + r.
    \label{eq:costafemheat}
\end{equation}
Likewise, the corrected equation for elasticity reads
\begin{equation}
    (A+M) U^{(i)} = F^{(i)} + 2M U^{(i-1)} - M U^{(i-2)} + r.
    \label{eq:CoSTA_elasticity}
\end{equation}    
As the boundary values are known, we do not need any correction for these elements.
Therefore the DDM only need to output values for the inner nodes.

In combining a PBM and a DDM, CoSTA aims to combine the strengths of both of these,
but it is clear that it also inherits weaknesses from both. It requires both a physical description of the system it models, as well as empirical data.
It needs to be trained before it can be used, but it also uses much computational resources to make a prediction, as two steps must be made with the PBM for every step with the CoSTA, in addition to the DDM prediction.
On the other hand, it is affected less by inaccuracy in the physical description than a PBM, and due to the minor role of the DDM part compared to a pure DDM method, it should also be less affected by poor quality or quantity of data. Finally, the extra accuracy it has shown easily justifies the additional computational cost.

==> junk/sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


